Inertia suppresses signatures of activity of active Brownian particles in a harmonic potential

A harmonically trapped active Brownian particle exhibits two types of positional distributions -- one has a single peak, the other has a single well -- that signify steady-state dynamics with low and high activity, respectively. Adding inertia to the translational motion preserves this strict single peak/well classification of the densities but shifts the dividing boundary between the states in the parameter space. We characterize this shift for the dynamics in one spatial dimension using the static Fokker--Planck equation for the full joint distribution of the state space. We derive local results analytically with a perturbation method for a small rotational velocity and then extend them globally with a numerical approach

==> Activity Threshold/mymacros.tex <==
%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%
\usepackage{amssymb,amsthm,amsmath,amsopn}
\usepackage[normal]{subfigure}
\usepackage{import}
\usepackage{verbatim}
\usepackage{mathrsfs}
\usepackage{colonequals}
\usepackage{paralist}
\usepackage{ctable}
\usepackage{bm}
\usepackage{mathtools}
\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}%
\usepackage{microtype}

%%%%%%%%%%%%%% IMAGES %%%%%%%%%%%%%%
\graphicspath{{./images/}}


%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{pr}{Principal Result}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{xca}[theorem]{Exercise}
\newtheorem{conj}[theorem]{Conjecture} 


\theoremstyle{definition}
\newtheorem*{definition}{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{unremark}{Remark}
\newtheorem*{example}{Example}
\newtheorem{problem}{Problem}
\newtheorem{hypothesis}[theorem]{Hypothesis}


%%%%%%%%%%%%%% FONTS %%%%%%%%%%%%%%
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}

%%%%%%%%%%%%%% LANDAU SYMBOLS %%%%%%%%%%%%%%
\newcommand{\bigoh}{\mathcal{O}}
\newcommand{\littleoh}{ \mbox{{\scriptsize $\mathcal{O}$}}}


%%%%%%%%%%%%%% ABBRS %%%%%%%%%%%%%%
\newcommand{\nn}{\nonumber}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{align}}
\newcommand{\eea}{\end{align}}
\newcommand{\bead}{\begin{aligned}}
\newcommand{\eead}{\end{aligned}}
\newcommand{\bsub}{\begin{subequations}}
\newcommand{\esub}{\end{subequations}}
\newcommand{\vect}[1]{\bm{#1}}
\newcommand{\clos}[1]{\bar{#1}}
\newcommand{\ds}[0]{\displaystyle}
\newcommand{\bs}[0]{\bm}
\def\grad{\nabla} 


\newcommand{\ce}{\colonequals}
\newcommand{\ec}{\equalscolon}
\newcommand{\til}[1]{\tilde{#1}}
\newcommand{\wtil}[1]{\widetilde{#1}}
\newcommand{\calig}[1]{\mathscr{#1}}
\newcommand{\re}[1]{\mathrm{Re}\left\{ #1\right\}}
\newcommand{\im}[1]{\mathrm{Im}\left\{ #1\right\}}
\newcommand{\tran}{^T} %{^{\mathstrut\top}} 
\DeclareMathOperator{\lintran}{\mathscr{L}}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\V}{vec}

\newcommand{\eqrefMLp}[2]{(\ref{#1}#2)} 
\newcommand{\eqrefMLnp}[2]{\ref{#1}#2}
%%% ejam multiline ref equations
% \newcommand{\eqrefMLp}[2]{$(\ref{#1}\,#2)$}
% \newcommand{\eqrefMLnp}[2]{$\ref{#1}\,#2$}


%%%%%%%%%%%%%% SPACES %%%%%%%%%%%%%%
\newcommand{\stsp}{\:\!}
\newcommand{\tsp}{\;\!}
\newcommand{\stnsp}{\!\!\:}
\newcommand{\ssp}[1]{{#1 \stnsp}}

%%%%%%%%%%%%%% DERIVATIVES %%%%%%%%%%%%%%
\newcommand*{\diff}{\mathop{}\!{d}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pddm}[3]{\frac{\partial^2 #1}{\partial #2 \hspace{1pt} \partial #3}}
\newcommand{\D}[2]{\frac{\diff #1}{\diff #2}}
\newcommand{\Dn}[3]{\frac{\diff^{#3} #1}{\diff #2^{#3}}}



%%%%%%%%%%%%%% GREEK %%%%%%%%%%%%%%
\newcommand{\eps}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\lam}{\lambda}
\newcommand{\gam}{\gamma}
\newcommand{\Lam}{\Lambda}

%%%%%%%%%%%%%% RULERS FOR TABLE %%%%%%%%%%%%%%%%
\newcommand{\otoprule}{\midrule [\heavyrulewidth]}





==> Activity Threshold/preamble.tex <==
%%%%% title, section, abstract, keywords  %%%%

\usepackage{titlesec}


\newcommand{\titleauthor}[2]{
	\hphantom{.}
	\vspace{.5in}
	\begin{center}
		\textbf{\Large \uppercase{#1}}
	\end{center}
	\begin{center}
		{\small \uppercase{#2}}
	\end{center}}
	
\newcommand{\ab}[1]{
	\vspace{-.15in}
	\begin{center}
		{\footnotesize \textbf{Abstract.}~{#1}}
	\end{center}
	\vspace{0in}}
	
\newcommand{\kw}[1]{
	\vspace{0in}
	\noindent\quad{\footnotesize \textbf{Keywords.}~{#1}}\\
	\vspace{0in}}
	
\newcommand{\amssub}[1]{
	\vspace{0in}
	\noindent\quad{\footnotesize \textbf{AMS subject classifications.}~{#1}}\\
	\vspace{0in}}

\titleformat{\title}[hang]{\large\bfseries}{}{0em}{\LARGE\bfseries}[]
\titleformat{\section}[hang]{\bf}{\thesection.}{.5em}{}[]
\titleformat{\subsection}[hang]{\it}{\thesubsection.}{.5em}{}[]
\titleformat{\subsection}[hang]{\it}{\thesubsection.}{.5em}{}[]
\titleformat{\subsubsection}[hang]{\it}{\thesubsubsection.}{.5em}{}[]
